A Traffic Control Framework for Uncrewed Aircraft Systems

The exponential growth of Advanced Air Mobility (AAM) services demands assurances of safety in the airspace. This research a Traffic Control Framework (TCF) for developing digital flight rules for Uncrewed Aircraft System (UAS) flying in designated air corridors. The proposed TCF helps model, deploy, and test UAS control, agents, regardless of their hardware configurations. This paper investigates the importance of digital flight rules in preventing collisions in the context of AAM. TCF is introduced as a platform for developing strategies for managing traffic towards enhanced autonomy in the airspace. It allows for assessment and evaluation of autonomous navigation, route planning, obstacle avoidance, and adaptive decision making for UAS. It also allows for the introduction and evaluation of advance technologies Artificial Intelligence (AI) and Machine Learning (ML) in a simulation environment before deploying them in the real world. TCF can be used as a tool for comprehensive UAS traffic analysis, including KPI measurements. It offers flexibility for further testing and deployment laying the foundation for improved airspace safety - a vital aspect of UAS technological advancement. Finally, this papers demonstrates the capabilities of the proposed TCF in managing UAS traffic at intersections and its impact on overall traffic flow in air corridors, noting the bottlenecks and the inverse relationship safety and traffic volume.

==> Discuss/Aaditya.tex <==
\subsection{Aaditya's Doubts}
\subsubsection{Environment Rules}
The TCF implements environment rules within the Air Corridor Model to govern the behavior of Unmanned Aerial Vehicles (UAVs) operating within this framework, ensuring the utilization of safety, reliability, and predictability. The following rules are applied to enable the effective use of the AirCorridor Model:

\begin{enumerate}
    \item \textbf{Safety Gap between UAVs:} It is required that each UAV maintains a minimum gap of at least 1 Air Cell when traveling within the same air lane. This rule guarantees that each vehicle has sufficient space to stop and recalibrate in the event of a malfunction or stoppage of the UAV ahead.
    \item \textbf{Broadcasting Information:} All UAVs are obligated to broadcast basic position information and a unique identifier at predetermined intervals. This rule aligns with existing regulations set by the Federal Aviation Administration (FAA) for UAVs flying in most airspaces.
    \item \textbf{Single Occupancy of Air Cells:} No Air Cell is allowed to accommodate more than one drone simultaneously. This rule ensures that there is no congestion or conflict within each discrete unit of airspace.
    \item \textbf{Intersection Dynamics:} The intersection of two Air Corridors creates a "directionless" space that does not impose any specific restrictions on the direction of UAV travel. This allows UAVs the opportunity to change their direction and enter a different air lane, which may belong to a different Air Corridor.
    \item \textbf{Locked Intersections:} In this version of the TCF, an intersection is considered "locked" when a drone occupies it. Only one drone is permitted within an intersection at any given time. Consequently, a drone can only enter an intersection when it is not locked, ensuring safe and orderly traffic within the intersection.
\end{enumerate}

By adhering to these rules within the Air Corridor Model, UAVs can navigate the airspace in a regulated and coordinated manner, ensuring efficient and secure operations. These rules are only applicable to TCF v1 and may change in future versions. \\ 
\hrule 

\hrule
\textcolor{green}{Note to self: The following paras are better suited in the Future work section}
Environmental adaptation is a crucial aspect of theTCF. The first version of TCF presented in this paper exclusively caters to discrete, deterministic, and fully observable environments. Under this framework, UAS operations can interact with the environment without encountering failures, whether it involves sensing or executing actions within the environment. 

However, future iterations of the TCF will expand its capabilities to encompass continuous and stochastic environments. The TCF will be enhanced to address the challenges associated with complex, dynamic, and uncertain environments, where continuous variables and stochastic processes play significant roles. This evolution of the TCF will allow for more realistic and versatile deployment of UAS in real-world scenarios, in applications ranging from surveillance and inspection to environmental monitoring and disaster response.\\
\hrule
\textcolor{green}{Note to self: The following paras are better suited in the Future work section}
However a more sophisticated method involves leveraging advanced AI/ML models. Through techniques such as Q-Learning, the agents can learn optimal decision-making policies and adapt their behavior over time. Unlike the strict, deterministic nature of the rules-based approach, this method allows agents to evolve and improve their decision-making capabilities based on their experiences and the feedback they receive from the environment.\\
\hrule
\textcolor{green}{Note to self: The following paras are better suited in the Future work section}
Future versions of TCF will allow for a support for a wide variety of sensor inputs as well as actions that are continuous and markovian, allowing for better environments.\\
\hrule
\textcolor{green}{Note to self: Need to find a place to fit the description of the abstraction layer}
The TCF serves as an effective tool to establish and promote uniformity across diverse UAS designs and functionalities. It accomplishes this by introducing a layer of abstraction over the specific operational details pertaining to individual UASs, their environment and their actions. 

The TCF's abstraction mechanism enables individual UAS attributes to be expressed in a cohesive and common language, independent of their specific makes or models. This abstraction oversees functions such as UAV movement, sensor outputs, operational states, and control inputs. As a result, unique UAV capabilities, constraints, and protocols are translated into a standardized format that can be comprehended and managed uniformly across all systems. 

==> Discuss/Abhiram.tex <==
\subsection{Abhiram's Doubts}

==> Discuss/Ananay.tex <==
\subsection{Ananay's Doubts}



==> Discuss/Ansh.tex <==
\subsection{Ansh's Doubts}

==> Discuss/Discuss.tex <==
\section{Discussions}
In this section, place all the doubts and suggestions you have. Wherever you have removed the para, please state the reason in \textcolor{red}{RED}. If possible, in lieu of the paragraphs under discussion please place your suggestions so that the suggestion can be seen with context. \\
This is so that all our doubts are stated clearly and at a common place

\input{Discuss/Ananay}
\input{Discuss/Aaditya}
\input{Discuss/Ansh}
\input{Discuss/Abhiram}

==> sections/TCF/communication_fabric.tex <==
\subsection{Communication Fabric}
The proposed \acrshort{tcf} abstracts this implementation of vehicle-to-vehicle communication by defining a communication fabric through which packets of data can be dispatched; conforming to prerequisites defined in \cref{sec:uav pre-req}


==> sections/TCF/env_sensing.tex <==
\subsection{Environment Sensing and Situational Awareness}
Environment sensing is extremely crucial in a dynamic setting such as air corridors. To the extent of this paper, environment sensing refers to the ability of the \acrshort{uav} to observe the traffic ahead. In particular, the distance/gap must be quantified which enables to check for any safety gap violation. Such knowledge of the environment is also required to determine the occupancy/vacancy of the intersection. 

This level of situational awareness allows for a unified perception of the environment across different \acrshort{uas}, enhancing their ability to cooperatively and independently react to changes in their operating environment. Hence through \acrshort{tcf}, consistent and predictable interactions between \acrshort{uav}s and their surroundings are achieved. 



==> sections/TCF/failure_management.tex <==
\subsection{Failure Management}
Presently, if a single UAS fails to adhere to the rules defined above, the entire system is considered to have failed. This is reflected in the following section where the simulation shuts down if a rule of the environment is not adhered to. 


==> sections/limitations.tex <==
\section{Limitations}
The current TCF model uses a binary probability distribution mechanism for traffic generation, however, more complex models will be implemented. 
In the initial iteration of the TCF, discrete, deterministic, and fully observable environments are utilized. However, in the second version we propose the incorporation of a continuous, stochastic environment to analyze dynamic and uncertain scenarios. This will allow for error prone and non ideal environments where data loss in the communication fabric, incorrect perception of the environment or an incorrect action taken by a UAS are considered.
A support for a wide variety of sensor inputs as well continuous and Markovian actions will also be included, further improving the environment perception of the UAVs. By introducing these changes, we aim to enhance the adaptability and effectiveness of the TCF in handling diverse and unpredictable environments. 

Furthermore, TCF is currenlty limited to 2 dimensional environments, which does not allow for certain traffic strategies to be tested. For example, having a bridge is a lot easier in 3 dimensions since the UAS can simply change altitude, which is not something the TCF allows in 2 dimensions. 
This support will also enhance the versatility of the TCF.

==> sections/simulation/deadlock.tex <==
\subsection{Deadlock}
  Deadlock (no drone passes through the intersection) which was introduced artificially to show how \acrshort{tpi}s would measure in that situation.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.40\textwidth]{Images/Deadlock-Sim.png}
    \caption{Deadlock Simulation}
    \label{fig:deadlock-sim}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.48\textwidth]{Images/Deadlock-Graph.png}
    \caption{Deadlock Graph}
    \label{fig:deadlock-graph}
\end{figure}

==> sections/simulation/distributed_queue_solution.tex <==
\subsection{Distributed Queue Solution}\
The Distributed Queue mechanism is an active decentralized queue that each \acrshort{uav} computes at an intersection. This queue mechanism was calculated by collecting data from each \acrshort{uav} as they broadcast information every simulation iteration. Each \acrshort{uav} had to compute its position on a queue, based on its distance from the intersection and its time spent waiting at the intersection and as a tie-breaker - in case the above two factors are identical - its unique identifier. This would give each \acrshort{uav} a unique position on the queue, and only the \acrshort{uav} at index 0 on the queue could traverse into the intersection and travel along the path. The first \acrshort{uav} on the queue is only allowed into the intersection if the intersection is not occupied.

This queue-based mechanism is easy to implement but is not the most reliable, since it requires efficient packet delivery of each \acrshort{uav}’s broadcast about its position details to all other \acrshort{uav}s, and this is not possible in the real world. In case a packet is dropped for even one \acrshort{uav} nearing the intersection it will change that \acrshort{uav}’s computation of the queue and might lead to issues. This mechanism has to be coupled with other safety protocols to prevent such edge cases from causing two \acrshort{uav}s to collide in the airspace. 

Apart from the performance guidelines, this queue based mechanism makes the following assumptions:
\begin{enumerate}
    \item The area of the \acrshort{uav} is negligible to the area of the entire Air Cell.
    \item The \acrshort{uav} knows its destination and path.
    \item All \acrshort{uav}s in the simulation are controlled by the same \acrshort{tcf} agent.
\end{enumerate}

Based on these assumptions, the following is set into force
\begin{enumerate}
    \item When the current \acrshort{uav} enters a threshold Air Cell in the intersection, it will listen for RID data from all \acrshort{uav}s in that threshold distance at all lanes from that intersection.
    \item The threshold is with respect to the center of intersection.
    \item \acrshort{uav}s listen to the environment and get RID data.
    \item \acrshort{uav}s compute the state of intersection from RID data.
    \item \acrshort{uav}s compute the queue of the intersection from RID data, and only consider \acrshort{uav}s traveling towards the intersection.
    \item The queue prioritizes vehicles based on priority (e.g. ambulance vs. passenger), time to intersection, and as a tiebreaker, \acrshort{uav} ID.
    \item When the \acrshort{uav} is at the top of the queue, and the intersection is open, the \acrshort{uav} enters the intersection.
    \item If 2 Aircells ahead of the current \acrshort{uav} have another \acrshort{uav}, the current \acrshort{uav} halts till the spot is free.
\end{enumerate}

The entire distributed queue mechanism is simple to implement within the \acrshort{tcf}. Each \acrshort{uav} will have a controlling agent that is called at every iteration of the simulation. This agent will get a context of the current environment, which includes access to the packets that were broadcast by other \acrshort{uav}s into the environment, or the \acrshort{uav}'s own speed and position. The underlying framework for acquiring these values is abstracted from the user, and in this case, is provided by our simulation. 

The \acrshort{uav} Agent will just have to report an Action that the \acrshort{uav} it is controlling needs to take. This is where the above rules are implemented given on the \acrshort{uav}'s state in the environment. Currently, due to the ideal nature of this particular use case, these rules will determine an optimal policy for all \acrshort{uav}'s to follow at the simulation. However future uses of \acrshort{tcf} can see the use of more advanced approaches to determine optimal policies based on these rules. 

The Python Code that is used in the \acrshort{uav} Agent can be verified using \acrshort{tcf} and then used as is in a \acrshort{uav} provided that the underlying driver code for the sensors and the control unit of the \acrshort{uav} provides all the capability that the \acrshort{tcf} agent expects. The developer's work then is reduced to just creating the bridge functions to provide the \acrshort{uav}'s environment context and the appropriate control logic for the actions that can be performed by the Agent.



==> sections/simulation/high-traffic.tex <==


When the traffic generation is set to more than 0.25, traffic congestion is never present. \Cref{fig:low-cong-sim} shows a visual representation of non-congested traffic. 

This is still a low traffic generation rate, however it is congesting since the bottleneck is 0.25 and the generation rate can be maximum up to 0.3. This will gradually cause a build up of drones in the system till there is a congestion.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.40\textwidth]{Images/Low-Congested-Sim.png}
    \caption{Low Congested Simulation}
    \label{fig:low-cong-sim}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.48\textwidth]{Images/Low-Non-Congested-Graph.png}
    \caption{Low Non-Congested Graph}
    \label{fig:low-non-cong-graph}
\end{figure}


\begin{comment}
    
High – Congestion: This is a high traffic generation rate of 0.8, which definitely causes congestion. The TPIs at this rate currently look similar to the Low – Congestion case since once the system is congested it is performing the same (all lanes filled with drones till the intersection, and only one lane with a drone exiting at a time). However I am not currently sure how it affects metrics we have not measured yet.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.40\textwidth]{Images/High-Congested-Sim.png}
    \caption{High Congested Simulation}
    \label{fig:high-cong-sim}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.48\textwidth]{Images/High-Congested-Graph.png}
    \caption{High Congested Graph}
    \label{fig:high-cong-graph}
\end{figure}

\end{comment}
    


==> sections/simulation/result.tex <==
\subsection{Results }

==> sections/simulation/simulating_on_tcf.tex <==
The TCF provides a standardization that cen be implemented programatically to serve as a simulation. As explored by this paper, we will attempt to find optimal policies for navigating a single intersection in the airspace by simulating drones on the TCF.

The simulation results presented in this paper were implemented in the Python Programming language. The various components such as agents and air corridors were their own python class keeping track of their respective attributes. 

The simulation had a basic control mechanism built in to allow for controlling speed. A map parser was also built to allow multiple maps to be loaded into the simulation and allow for changing the environment in which the drones are being simulated.

==> sections/simulation/single_intersection_model.tex <==
\subsection{Single Intersection Model}




 


==> sections/structured_airspace/need_for_structured_airspaces.tex <==


